SUMMIT: Source-Free Adaptation of Uni-Modal Models to Multi-Modal Targets

Scene understanding using multi-modal data is necessary in many applications, e.g., autonomous navigation. To achieve this in a variety of situations, existing models must be able to adapt to shifting data distributions without arduous data annotation. Current approaches assume that the source data is available during adaptation and that the source consists of paired multi-modal data. Both these assumptions may be problematic for many applications. Source data may not be available due to privacy, security, or economic concerns. Assuming the existence of paired multi-modal data for training also entails significant data collection costs and fails to take advantage of widely available freely distributed pre-trained uni-modal models. In this work, we relax both of these assumptions by addressing the problem of adapting a set of models trained independently on uni-modal data to a target domain consisting of unlabeled multi-modal data, without having access to the original source dataset. Our proposed approach solves this problem through a switching framework which automatically chooses between two complementary methods of cross-modal pseudo-label fusion -- agreement filtering and entropy weighting -- based on the estimated domain gap. We demonstrate our work on the semantic segmentation problem. Experiments across seven challenging adaptation scenarios verify the efficacy of our approach, achieving results comparable to, and in some cases outperforming, methods which assume access to source data. Our method achieves an improvement in mIoU of up to 12% over competing baselines. Our code is publicly available at https://github.com/csimo005/SUMMIT.

==> sections/temp.tex <==
While xMUDA~\cite{jaritz2020xmuda} has made significant improvements over unimodal UDA methods, it assumes that the source dataset used for training (i) consists of paired multi-modal data, and (ii) is available during adaptation to the target domain. However, these conditions may be hard to satisfy in real world scenarios. \\
- The first assumption is problematic because the availability of paired data may not be guaranteed, for example, in cases where sensor synchronization is poor, data stream frame rate may vary/drop over time, or when data for each sensing modality are captured separately. It would also require separately trained source models to be retrained on paired data before adaptation, which is quite impractical.
- The second assumption is problematic because sharing the source data for adaptation purposes may be impossible due to privacy or security concerns, or impractical due to costs of storing and sharing the entire source dataset. \\
Relaxing the first assumption of paired modalities in the source domain remains unaddressed in cross-modal UDA. The second assumption has been relaxed in the source-free UDA setting, but to the authors' best knowledge, no such prior works deal with multi-modal data~\cite{liang2020we,ahmed2021unsupervised,yeh2021sofa,xia2021adaptive}. 

In this paper, we perform \textit{\underline{S}ource-free Adaptation of \underline{U}nimodal models to \underline{M}ulti-\underline{M}odal \underline{T}argets} (SUMMIT), relaxing both assumptions of the xMUDA setting simultaneously (see Figure~\ref{fig:teaser}). Relaxation of the two assumptions in conventional cross-modal UDA, makes our problem substantially more challenging.
In the conventional cross-modal UDA setting, the approach in~\cite{jaritz2020xmuda} leverages labeled paired multi-modal data to learn correlations across modalities. This correlation is then used to improve transfer to the target domain. In our case, the correlations between modalities must be learned on the unsupervised target data since we do not assume access to such labeled pairs. The lack of source data already makes the alignment of the source and target distributions challenging. The combined relaxation of both assumptions makes the overall problem even more challenging.

==> tables/ablation_AF.tex <==
\begin{table}[t]
    % \small
    \centering
    \caption{We examine the interplay between agreement filtering (AF), entropy weighting (EW), hypothesis testing (HT), and the cross-modal loss $\mathcal{L}_{xM}$. We note that both AF and EW on their own provide an improvement across modalities and works well with the cross-modal loss. HT provides some benefit for the 2D modality and a definite improvement for 2D+3D for AF, and a large improvement on the fused 2D+3D output for EW in both the USA/Singapore and the Day/Night adaptation scenarios.however this comes as the expense of the 3D modality. However, it hurts performance on the A2D2/SemanticKITTI adaptation scenario, which we explore further in Section~\ref{experiments:pl_accuracy}.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccccccccc}
      \toprule
       & \multicolumn{3}{c}{USA/Singapore} & \multicolumn{3}{c}{Day/Night} & \multicolumn{3}{c}{A2D2/SemKITTI}\\
      \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
      Method & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D \\
      \midrule
      No Adaptation & 49.27 & 51.14 & 55.66 & 29.83 & 41.20 & 34.70 & 35.36 & 36.21 & 43.07\\
      \midrule
      AF & 53.53 & 53.44 & 56.60 & 33.06 & 42.55 & 35.45 & 47.15 & 50.96 & 51.26\\
      AF+$\mathcal{L}_{xM}$ & 54.64 & 53.14 & 57.22 & 39.24 & 42.48 & 41.25 & 47.57 & 51.01 & 51.38\\
      AF+HT & 55.29 & 52.11 & 61.49 & 36.58 & 38.45 & 40.11 & 35.78 & 36.09 & 37.93\\
      AF+HT+$\mathcal{L}_{xM}$ & 55.52 & 52.26 & 61.36 & 37.59 & 38.38 & 41.08 & 35.66 & 36.14 & 37.79\\
      \midrule
      EW & 55.37 & 54.20 & 58.67 & 33.83 & 42.23 & 35.32 & 41.66 & 46.27 & 45.80 \\
      EW+$\mathcal{L}_{xM}$ & 56.30 & 54.12 & 59.43 & 39.16 & 42.04 & 40.44 & 41.74 & 46.31 & 45.85 \\
      EW+HT & 55.70 & 53.33 & 62.22 & 39.94 & 41.69 & 43.56 & 38.50 & 43.87 & 42.22 \\
      EW+HT+$\mathcal{L}_{xM}$ & 55.87 & 53.47 & 62.19 & 40.98 & 41.54 & 44.83 & 38.46 & 43.87 & 42.16\\
      \midrule
      Oracle & 61.73 & 56.52 & 69.36 & 45.74 & 43.73 & 49.54 & 64.77 & 72.95 & 75.06\\
      \bottomrule
    \end{tabular}\label{tab:ablation_AF}
}
\end{table}

% Experiment numbers
% USA/Singapore
% 83176
% 81599
% 83518
% 83513
% 83497
% 83474
% 83531
% 83519
% DAY/NIGHT
% 83326, 83450
% 81600
% 83574
% 83535
% 83510
% 83488
% 83563
% 83562
% A2D2/SemanticKITTI
% 83455
% 81601
% 83577
% 83578
% 83489
% 83496
% 83551
% 83552

==> tables/ablation_AF_EW.tex <==
\begin{table}
    \centering
    \caption{Here we examine the effect of each loss term on the mIoU for each adaptation scenario. Here AF is an abbreviation for agreement filtering, the method used to combine pseudo labels across modalities, and HT is abbreviation for hypothesis testing. We note that while each successive component tends to build positively on the others and that while the loss functions do improve performance, our method of combining pseudo labels across modalities provides a large improvement over the baseline on its own.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{*{10}{lccccccccc}}
      \toprule
       & \multicolumn{3}{c}{USA/Singapore} & \multicolumn{3}{c}{Day/Night} & \multicolumn{3}{c}{A2D2/SemanticKITTI}\\
      \cmidrule(lr){2-5}\cmidrule(l{2.5\tabcolsep}r{.25\tabcolsep}){5-7}\cmidrule(l{.25\tabcolsep}r{.25\tabcolsep}){7-10}
      Method & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D \\
      \midrule
      Baseline & 49.27 & 51.14 & 55.66 & 29.83 & 41.20 & 34.70 & 35.36 & 36.21 & 43.07\\
      \midrule
      AF+EW & & - & - & - & - & - & - & - & - & -\\
      AF+EW+$\mathcal{L}_{xM}$ & 55.94 & 53.93 & 58.96 & - & - & - & - & - & -\\
      AF+EW+HT & - & - & - & - & - & - & - & - & -\\
      AF+EW+HT+$\mathcal{L}_{xM}$ & 55.94 & 53.94 & 58.96 & - & - & - & - & - & -\\
      \midrule
      Oracle & 61.73 & 56.52 & 69.36 & 45.74 & 43.73 & 49.54 & 64.77 & 72.95 & 75.06\\
      \bottomrule
    \end{tabular}\label{tab:abalation_AF}
}
\end{table}

% Experiment numbers
% USA/Singapore
% 83530
% 83508
% 83523
% 83509
% DAY/NIGHT
% 
% 
%
%
% A2D2/SemanticKITTI
% 
% 
%
%

==> tables/ablation_EW.tex <==
\begin{table}
    \centering
    \caption{Here we examine the interplay between entropy weighting (EW), hypothesis testing (HT), and the cross-modal loss $\mathcal{L}_{xM}$. The baseline method is the unadapted source model and oracle is the source model adapted with ground truth labels on target. We see that entropy weighting also provides a significant improvement on its own. Hypothesis testing gives a large improvement on the fused 2D+3D output in both the USA/Singapore and the Day/Night adaptation scenarios. Similar to agreement filtering we see that hypothesis testing hurts performance on the A2D2/SemanticKITTI adaptation scenario.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{*{10}{lccccccccc}}
      \toprule
       & \multicolumn{3}{c}{USA/Singapore} & \multicolumn{3}{c}{Day/Night} & \multicolumn{3}{c}{A2D2/SemanticKITTI}\\
      \cmidrule(lr){2-5}\cmidrule(l{2.5\tabcolsep}r{.25\tabcolsep}){5-7}\cmidrule(l{.25\tabcolsep}r{.25\tabcolsep}){7-10}
      Method & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D \\
      \midrule
      Baseline & 49.27 & 51.14 & 55.66 & 29.83 & 41.20 & 34.70 & 35.36 & 36.21 & 43.07\\
      \midrule
      EW & 55.37 & \underline{54.20} & 58.67 & 33.83 & \underline{42.23} & 35.32 & 41.66 & 46.27 & 45.80 \\
      EW+$\mathcal{L}_{xM}$ & \underline{56.30} & 54.12 & 59.43 & 39.16 & 42.04 & 40.44 & \underline{41.74} & \underline{46.31} & \underline{45.85} \\
      EW+HT & 55.70 & 53.33 & \underline{62.22} & 39.94 & 41.69 & 43.56 & 38.50 & 43.87 & 42.22 \\
      EW+HT+$\mathcal{L}_{xM}$ & 55.87 & 53.47 & 62.19 & \underline{40.98} & 41.54 & \underline{44.83} & 38.46 & 43.87 & 42.16\\
      \midrule
      Oracle & 61.73 & 56.52 & 69.36 & 45.74 & 43.73 & 49.54 & 64.77 & 72.95 & 75.06\\
      \bottomrule
    \end{tabular}\label{tab:ablation_EW}
}
\end{table}

% Experiment numbers
% USA/Singapore
% 83497
% 83474
% 83531
% 83519
% DAY/NIGHT
% 83510
% 83488
% 83563
% 83562
% A2D2/SemanticKITTI
% 83489
% 83496
% 83551
% 83552

==> tables/adaptation_std.tex <==
\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{cccccc}
        \toprule
        \multicolumn{3}{c}{\textbf{A2D2/SemKITTI}} & \multicolumn{3}{c}{\textbf{(Day2D,Night3D)/SemKITTI}}\\
        \cmidrule(lr){1-3}\cmidrule(lr){4-6}
        2D & 3D & 2D+3D & 2D & 3D & 2D+3D \\
        \midrule
        $44.67\pm 0.30$ & $48.56\pm0.33$ & $49.93\pm0.13$ & $32.19\pm 0.23$ & $38.71\pm 0.27$ & $35.51\pm 0.16$\\
        \bottomrule
    \end{tabular}\label{tab:std}
    }
\end{table}

% Experiment numbers
% 81601
% 139432
% 139438

==> tables/cross_entropy_ablation.tex <==
\begin{table}[t]
    \centering 
    \tiny
    \caption{Our estimated weights provides a significant improvement over the unweighted cross-entropy loss.}    
   % \resizebox{0.85\columnwidth}{!}{
    \begin{tabular}{lccc}
      \toprule
       &  \multicolumn{3}{c}{\textbf{USA/Singapore}}\\
      \cmidrule(lr){2-4}
      \textbf{Method} & 2D & 3D & 2D+3D\\
      \midrule\
        Unweighted & 49.97 & 45.11 & 51.47\\
        Weighted  & \textbf{57.47} & \textbf{52.12} & \textbf{62.32}\\
      \bottomrule
    \end{tabular}
    \label{tab:ce_ablation}
   % }
\end{table}

==> tables/crossover_expanded_pl_accuracy.tex <==
% \begin{table*}[t]
%     \centering
%     \caption{} 
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lcccccccccccccc}
%       \toprule
%        & \multicolumn{3}{c}{\textbf{(USA-2D,Singapore-3D)/SemKITTI}} & \multicolumn{3}{c}{\textbf{(Singapore-2D,USA-3D)/SemKITTI}} & \multicolumn{3}{c}{\textbf{(Day-2D,Night-3D)/SemKITTI}} & 
%        \multicolumn{3}{c}{\textbf{(Night-2D,Day-3D)/SemKITTI}}\\
%       \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
%       \textbf{Method} & Correct & Incorrect & Ignore & Correct & Incorrect & Ignore & Correct & Incorrect & Ignore & Correct & Incorrect & Ignore\\
%       \midrule
%       AF & 28.66 &  3.23 & 68.11 & 30.78 &  3.38 & 65.84 & 32.76 &  4.77 & 62.46 & 26.44 &  3.19 & 70.37\\
%       EW & 4.18 & 78.66 & 15.16 & 3.43 & 86.78 & 9.79 & 3.46 & 86.26 & 10.28 & 1.36 & 94.59 & 3.71\\
%       EW + HT &  7.49 & 85.28 &  7.23 &  4.26 & 89.92 &  5.82 &  4.41 & 89.97 &  5.62 &  1.41 & 94.88 &  3.71\\
%       \bottomrule
%     \end{tabular}\label{tab:crossover_filtering}
% }
% \end{table*}
\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccccccc}
      \toprule
       & \multicolumn{3}{c}{\textbf{(USA-2D,Singapore-3D)/SemKITTI}} & \multicolumn{3}{c}{\textbf{(Singapore-2D,USA-3D)/SemKITTI}}\\
      \cmidrule(lr){2-4}\cmidrule(lr){5-7}
      \textbf{Method} & Correct & Incorrect & Ignore & Correct & Incorrect & Ignore\\
      \midrule
      EW & 4.18 & 78.66 & 15.16 & 3.43 & 86.78 & 9.79\\
      EW + HT &  7.49 & 85.28 &  7.23 &  4.26 & 89.92 &  5.82\\
      \bottomrule
    \end{tabular}\label{tab:crossover_filtering}
}
\end{table}

==> tables/crossover_filtering_half.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{Pseudo-label accuracy for crossover experiments.} In crossover experiments we see that AF correctly labels a much larger portion of admitted samples. In contrast EW admits many samples, but the pseudo-labels are generally incorrect. Our switching strategy correctly chooses AF in all these scenarios.} 
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccccccc}
      \toprule
       & \multicolumn{3}{c}{\textbf{(USA-2D,Singapore-3D)/SemKITTI}} & 
       \multicolumn{3}{c}{\textbf{(Night-2D,Day-3D)/SemKITTI}}\\
      \cmidrule(lr){2-4}\cmidrule(lr){5-7}
      \textbf{Method} & Correct & Incorrect & Ignore & Correct & Incorrect & Ignore\\
      \midrule
      AF & 28.66 &  3.23 & 68.11 & 26.44 &  3.19 & 70.37\\
      EW &  7.49 & 85.28 &  7.23 &  1.41 & 94.88 &  3.71\\
      \bottomrule
    \end{tabular}\label{tab:crossover_filtering}
}
\end{table}

==> tables/crossover_performance.tex <==
\begin{table*}[ht]
    \centering
    % \caption{In the crossover every adaptation method experiences a drop in perfromance, since this adaptation scenario has not only differences in sensor configuration and label distribution, but also has no possibility of existing correlations between methods. While our method is not an exception to this we see that we are still able to consistently improve over the unadapted source model and adaptation models. In some cases our adaptation is able to improve performance by as much as 12\%.} 
    \caption{\textbf{Results on crossover adaptation scenarios.} Differences in sensor configuration and label distribution result in all methods experiencing a drop in performance. While our method is not an exception to this, we obtain consistent improvements of up to 12\% over the unadapted source model and other adaptation approaches.} 
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lcccccccccccccc}
      \toprule
       &  &  & \multicolumn{3}{c}{\textbf{(USA-2D,Singapore-3D)/SemKITTI}} & \multicolumn{3}{c}{\textbf{(Singapore-2D,USA-3D)/SemKITTI}} & \multicolumn{3}{c}{\textbf{(Day-2D,Night-3D)/ SemKITTI}} & \multicolumn{3}{c}{\textbf{(Night-2D,Day-3D)/SemKITTI}}\\
      \cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}\cmidrule(lr){13-15}
      \textbf{Method} & \textbf{Multimodal} & \textbf{Source-free} & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D \\
      \midrule
      No adaptation & - & - & 18.98 & 28.94 & 26.77 & 20.22 & 28.45 & 25.51 & 24.21 & 28.54 & 29.96 & 16.14 & 26.60 & 20.52\\
      \midrule
      xMUDA SF & \cmark & \cmark & 16.94 & 33.85 & 27.35 & 20.38 & 32.38 & 28.25 & 24.55 & 33.96 & 29.43 & 16.11 & 28.00 & 25.90\\
      SHOT & \xmark & \cmark & 24.53 & 34.06 & 29.10 & 16.09 & 28.12 & 25.80 & 19.44 & 34.11 & 27.37 & 20.41 & 32.41 & 28.18\\
      \midrule
      Ours & \cmark & \cmark & \textbf{28.02} & \textbf{34.27} & \textbf{30.81} & \textbf{29.55} & \textbf{32.91} & \textbf{31.95} & \textbf{32.42} & \textbf{38.54} & \textbf{35.67} & \textbf{28.63} & \textbf{32.98} & \textbf{30.87}\\
      \midrule
      Oracle & - & - & 55.36 & 68.73 & 69.82 & 56.37 & 67.69 & 70.60 & 58.20 & 67.82 & 70.82 & 56.41 & 68.69 & 69.90 \\
      \bottomrule 
    \end{tabular}\label{tab:crossover_performance}
}
\end{table*}



==> tables/crossover_switching_half.tex <==
\begin{table}[t]
    \centering
    \caption{\textbf{Source \& target agreement for crossover  experiments.} In the crossover experiments, the source agreement is lower across the board. However, because of the large domain gap between the source and target, the target agreement is far lower as well. This results in AF being used for all the crossover experiments.} 
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcc}
      \toprule
       &  \textbf{(USA-2D, Singapore-3D)/SemKITTI} & \textbf{(Night-2D, Day-3D)/SemKITTI}\\
      \midrule
      Source Agreement & 86.37 & 75.09\\
      Target Agreement & 38.60 & 35.00\\
      \midrule
      Ratio & 0.45 & 0.47\\
      \bottomrule
    \end{tabular}\label{tab:crossover_switching}
}
\end{table}

==> tables/expanded_pl_accuracy.tex <==
% \begin{table*}[t]
%     \centering
%     \caption{} 
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lccccccccc}
%       \toprule
%        & \multicolumn{3}{c}{\textbf{USA/Singapore}} & \multicolumn{3}{c}{\textbf{Day/Night}} & \multicolumn{3}{c}{\textbf{A2D2/SemanticKITTI}}\\
%       \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
%       \textbf{Method} & Correct & Incorrect & Ignore & Correct & Incorrect & Ignore & Correct & Incorrect & Ignore\\
%       \midrule
%       AF & 87.29 & 0.13 & 12.58 & 88.45 & 0.10 & 11.45 & 23.76 & 1.73 & 74.51\\
%       EW & 89.67 & 0.33 & 10.00 & 93.35 & 0.30 & 6.45 & 39.51 & 11.54 & 48.94\\
%       EW + HT & 93.40 & 0.65 & 5.94 & 94.51 & 0.56 & 4.93 & 55.42 & 24.72 & 19.85\\
%       \bottomrule
%     \end{tabular}\label{tab:crossover_filtering}
% }
% \end{table*}

\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccccc}
      \toprule
       & \multicolumn{3}{c}{\textbf{USA/Singapore}} & \multicolumn{3}{c}{\textbf{A2D2/SemanticKITTI}}\\
      \cmidrule(lr){2-4}\cmidrule(lr){5-7}
      \textbf{Method} & Correct & Incorrect & Ignore & Correct & Incorrect & Ignore\\
      \midrule
      EW & 89.67 & 0.33 & 10.00 & 39.51 & 11.54 & 48.94\\
      EW + HT & 93.40 & 0.65 & 5.94 & 55.42 & 24.72 & 19.85
      % \bottomrule
    \end{tabular}\label{tab:crossover_filtering}
}
\end{table}

==> tables/performance.tex <==
\begin{table*}[ht]
    \centering
    \caption{\textbf{Results on primary adaptation scenarios.} Our framework outperforms both the uni-modal and multi-modal source-free adaptation baselines by a large margin across all scenarios. Note that xMUDA needs source data, and the results below are provided assuming that the source data is available during adaptation. Despite xMUDA requiring access to source data and models that are jointly trained on multi-modal data, our method has comparable performance and even outperforms it in the A2D2/SemanticKITTI scenario.} 
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccccc}
      \toprule
       &  &  & \multicolumn{3}{c}{\textbf{USA/Singapore}} & \multicolumn{3}{c}{\textbf{Day/Night}} & \multicolumn{3}{c}{\textbf{A2D2/SemKITTI}}\\
      \cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}
      \textbf{Method} & \textbf{Multimodal} & \textbf{Source-free} & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D \\
      \midrule
      No adaptation & - & - & 49.67 & 47.39 & 55.96 & 41.85 & 42.32 & 49.98 & 32.85 & 34.01 & 40.52\\
      xMUDA & \cmark & \xmark & 61.10 & 54.10 & 63.20 & 47.10 & 46.70 & 50.80 & 43.70 & 48.50 &  49.10\\
      \midrule
      xMUDA SF & \cmark & \cmark & 52.02 & 50.73 & 54.90 & 35.22 & 44.10 & 42.74 & 5.32 & 7.53 & 6.59\\
      SHOT & \xmark & \cmark & 52.21 & 48.20 & 58.18 & 34.68 & 40.61 & 40.82 & 33.52 & 36.95 & 42.28\\
      \midrule
      Ours & \cmark & \cmark & \textbf{57.47} & \textbf{52.12} & \textbf{62.32} & \textbf{44.73} & \textbf{44.53} & \textbf{50.72} & \textbf{45.01} & \textbf{48.34} & \textbf{49.96}\\
      \midrule
      Oracle & - & - & 64.67 & 57.19 & 71.29 & 46.11 & 40.31 & 45.60 & 58.84 & 71.75 & 74.57\\
      \bottomrule
    \end{tabular}\label{tab:performance}
}
\end{table*}

% Experiment numbers
% USA/Singapore
% 73301
% Copied from xmuda table
% 75988
% 82780
% 
% 76467
% DAY/NIGHT
% 76015
% Copied from xmuda table
% 76052
% 83014
%
% 81717
% A2D2/SemanticKITTI
% 76054
% Copied from xmuda tablemk
% 76067
% 83449
%
% 76569

==> tables/psuedo_label_recalculation.tex <==
\begin{table}[t]
    \centering 
    \tiny
    \caption{Frequent recalculation of pseudo-labels hurts our method, with the least frequent seeing a minor improvement on 3D only, compared to no recalculation shown in the last row.}     
   % \resizebox{0.85\columnwidth}{!}{
    \begin{tabular}{cccc}
      \toprule
       & \multicolumn{3}{c}{\textbf{USA/Singapore}}\\
      \cmidrule(lr){2-4}
      \textbf{Pseudo Label Period (Steps)} & 2D & 3D & 2D+3D\\
      \midrule
%      No adaptation & - & 49.67 & 47.39 & 55.96\\
%      \midrule
      10000 & 50.77 & 47.27 & 51.03\\
      20000 & 54.84 & 50.19 & 55.34\\
      50000 & 56.45 & \textbf{52.75} & 58.08\\
        N/A & \textbf{57.47} & 52.12 & \textbf{62.32}\\
%      \midrule
%      Oracle & - & 64.67 & 57.19 & 71.29\\
      \bottomrule
    \end{tabular}
    \label{tab:pl_recalc}
   % }
\end{table}
% Experiment numbers
% USA/Singapore
% 73301
% 81878
% 81879
% 81880
% 82780

==> tables/rebuttal_exp.tex <==
% \begin{table}[t]
\begin{wraptable}{l}{0.46\columnwidth}
    % \footnotesize
    \resizebox{0.55\columnwidth}{!}{
    % \caption{Here we compare the use of the median and the mean for determining the certainty threshold in agreement filtering. We see that median performs better across the board by at least 1-2\% and that the median performs much better with hypothesis testing down stream. This is likely due to some skewness in the distribution, since the arithmetic mean is known to be sensitive to outliers.}
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{lccc}
      \toprule
       & \multicolumn{3}{c}{USA/Singapore}\\
      \cmidrule(lr){2-4}
      Method & 2D & 3D & 2D+3D\\
      \midrule
      No Adaptation & 49.27 & 51.14 & 55.66\\
      \midrule
      AF, median & 54.64 & 53.14 & 57.22\\
      AF, mean & 54.21 & 51.01 & 55.80\\
      AF+HT, median & 55.29 & 52.26 & 61.36\\
      AF+HT, mean & 51.80 & 44.73 & 52.95\\
      \midrule
      Oracle & 61.73 & 56.52 & 69.36\\
      \bottomrule
    \end{tabular}\label{tab:rebuttal}
    }
% }
\end{wraptable} 
% \end{table}

==> tables/rebuttal_setting.tex <==
% \begin{table}[t]
\begin{wraptable}{l}{0.46\columnwidth}
    % \footnotesize
    \resizebox{0.54\columnwidth}{!}{
    \centering
    % \caption{Here we compare the use of the median and the mean for determining the certainty threshold in agreement filtering. We see that median performs better across the board by at least 1-2\% and that the median performs much better with hypothesis testing down stream. This is likely due to some skewness in the distribution, since the arithmetic mean is known to be sensitive to outliers.}
    % \resizebox{\columnwidth}{!}{
    \begin{tabular}{lcccc}
      \toprule
      \multicolumn{2}{c}{Source} & \multicolumn{3}{c}{USA/Singapore}\\
      \cmidrule(lr){1-2}\cmidrule(lr){3-5}
      Access & Paired & 2D & 3D & 2D+3D\\
      \midrule
      \cmark & \cmark & 61.10 & 54.10 & 63.20\\
      \xmark & \cmark & 57.50 & 54.97 & 60.38\\
      \xmark & \xmark & 50.60 & 53.75 & 53.75 \\
      %\midrule
      %Oracle & 61.73 & 56.52 & 69.36\\
      \bottomrule
    \end{tabular}\label{tab:rebuttal_setting}
    }
% }
\end{wraptable} 
% \end{table}

==> tables/settings.tex <==
% \begin{wraptable}{r}{0.55\textwidth}
\begin{table}[t]
    \centering
    \small
    \caption{We show how fusing pseudo-labels can help across different adaptation scenarios on the USA/Singapore scenario. While we see that incorporating does tend to help the individual data modalities, it causes a drop in the combine fused 2D+3D output. In settings which have access to source data, the additional loss terms may be making the models less focused.}
    % \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{lcccccc}
      \toprule
       & \multicolumn{3}{c}{Agreement Filtering} & \multicolumn{3}{c}{Entropy Weighting}\\
      \cmidrule(lr){2-4}\cmidrule(l{2.5\tabcolsep}r{.25\tabcolsep}){5-7}
      Setting & 2D & 3D & 2D+3D & 2D & 3D & 2D+3D \\
      \midrule
      SCUDA & 55.52 & 52.26 & 61.36 & 55.87 & 53.47 & 62.19 \\
      Multi-modal SF & 56.38 & 52.70 & 61.65 & 57.11 & 53.97 & 62.44 \\
      Unpaired Source UDA & 56.31 & 52.39 & 59.65 & 56.95 & 53.69 & 60.79 \\ 
      xMUDA & 56.60 & 53.15 & 59.62 & 57.37 & 53.82 & 60.57 \\ 
      \bottomrule
    \end{tabular}
    % }
    \label{tab:settings}
\end{table}
% \end{wraptable}

==> tables/unfiltered.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{We evaluate the correctness of pseudo-labels for each modality when only certainty filtering is done according to Eq.~\ref{eq:certainty_filter}. We note that while the 2D modality has a large proportion of correct labels, it typically contains more than double the amount of incorrect labels when compared with 3D. This helps to explain why it is easier to improve the 2D performance more than the 3D, since our framework removes more incorrect labels from the 2D modality.}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{*{10}{lccccccccc}}
      \toprule
       & \multicolumn{3}{c}{USA/Singapore} & \multicolumn{3}{c}{Day/Night} & \multicolumn{3}{c}{A2D2/SemKITTI}\\
      \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
      Modality & Correct & Incorrect & Ignore & Correct & Incorrect & Ignore & Correct & Incorrect & Ignore \\
      \midrule
      2D & 96.38 & 1.45 & 2.17 & 95.94 & 1.76 & 2.30 & 50.10 & 17.95 & 33.27\\
      3D & 89.13 & 0.65 & 10.22 & 90.67 & 0.45 & 8.88 & 44.70 & 11.68 & 46.06\\
      \bottomrule
    \end{tabular}\label{tab:unfiltered}
}
\end{table}
